Selected Chapters on Active Galactic Nuclei as Relativistic Systems

This volume presents an overview of selected aspects of physical processes occurring in the inner regions of Active Galactic Nuclei (AGN). The observational evidence suggests that strong gravitational fields play a significant role in governing the energy output of AGN and their influence on the surrounding medium, possibly due to the presence of a supermassive black hole. In order to reduce an unnecessary overlap with numerous reviews on the subject of AGN, here we focus on several selected topics.

==> babelbst.tex <==
%% $Id: babelbst.tex,v 0.3 2007/02/23 09:35:47 sta Exp $
%% The structure of this file depends on your language selection
%% in the `latex' and/or `pdflatex' format.  This can be achieved
%% by inspecting language file `language.dat' (typically location
%% is /var/lib/texmf/tex/generic/config/language.dat, but this
%% can vary from distro to distro).  Follow instruction in this
%% file and activate the languages required (US-English should
%% always be activated as the first, i.e., number 0 language).
%% Then re-generate the above formats.  The selected languages
%% are numbered starting from 0 (American English).  Check the
%% language enumeration by inspecting the format generation log
%% files latex.log and/or pdflatex.log (search for the string
%% \language).  Now, in the switch structure below, input
%% bibliography language definition (.bld) file belonging to
%% the language number as described above in the corresponding
%% branch of the `\ifcase' switch structure.  If required, feel
%% free to add further languages.  Good luck.
%%

\ifcase\language % 0=american(=USenglish)
  \input{american.bld}
\or % 1=british(=UKenglish=english)
  \input{british.bld}
\or % 2=french(=patois)
  \input{french.bld}
\or % 3=german(=austrian)
  \input{german.bld}
\or % 4=ngerman(=naustrian)
  \input{ngerman.bld}
\or % 5=czech
  \input{czech.bld}
\or % 6=slovak
  \input{slovak.bld}
\else % 7=nohyphenation
  \input{american.bld}
\fi

\endinput
%%
%% End of file `babelbst.tex'.

